DRILL-- Deep Reinforcement Learning for Refinement Operators in $\mathcal{ALC}$

Approaches based on refinement operators have been successfully applied to class expression learning on RDF knowledge graphs. These approaches often need to explore a large number of concepts to find adequate hypotheses. This need arguably stems from current approaches relying on myopic heuristic functions to guide their search through an infinite concept space. In turn, deep reinforcement learning provides effective means to address myopia by estimating how much discounted cumulated future reward states promise. In this work, we leverage deep reinforcement learning to accelerate the learning of concepts in $\mathcal{ALC}$ by proposing DRILL -- a novel class expression learning approach that uses a convolutional deep Q-learning model to steer its search. By virtue of its architecture, DRILL is able to compute the expected discounted cumulated future reward of more than $10^3$ class expressions in a second on standard hardware. We evaluate DRILL on four benchmark datasets against state-of-the-art approaches. Our results suggest that DRILL converges to goal states at least 2.7$\times$ faster than state-of-the-art models on all benchmark datasets. We provide an open-source implementation of our approach, including training and evaluation scripts as well as pre-trained models.

==> part7.tex <==
\section{Conclusion and Future Work}
\label{sec:conclusion}
%
In this work, we introduced \approach---a novel class expression learning approach that leverages a convolutional deep Q-network to accelerate the learning of concepts in \ALC.
% a class expression learning approach which uses a convolutional deep Q-learning model as heuristic function. 
To our knowledge, \approach is the first deep reinforcement model that is used to learn class expressions in $\mathcal{ALC}$. By virtue of using reinforcement learning, \approach is endowed with the capability of incorporating information pertaining to future rewards while determining the heuristic value of states. \ac{CEL} approaches lack this ability as they rely on myopic heuristic functions to guide their search through an infinite concept space. Our experiments show that \approach outperforms state-of-the-art approaches w.r.t. its runtime. Our statistical hypothesis test confirms the superior performance of \approach on all benchmark datasets.

In future work, we plan to investigate: 
\begin{inparaenum}[(i)]
\item learning embeddings during the training phase, 
\item using LSTM and Transformer architecture in \approach, 
\item constructing a reward function based the gain function in DL-FOIL, and 
\item leveraging  reinforcement learning at generating difficult learning problems.
\end{inparaenum}

==> tables/Carcinogenesis_results.tex <==
\begin{table*}[!t]
    \caption{Results of single learning problems on the Carcinogenesis benchmark dataset. Maximum runtime is set to 3 seconds. L, F1, Acc and T stand for length of the predicted class expression, F-measure, Accuracy and runtime in seconds. Learning problems are obtained from DL-learner.}
    % DOUBLE check the results and floating points.
    \centering
    \small
    \begin{tabular}{lccccccccccccccccccccc}
    \toprule 
      Targets & \multicolumn{4}{c}{\textbf{\approach}}&& \multicolumn{4}{c}{\textbf{CELOE}}&& \multicolumn{4}{c}{\textbf{OCEL}}&& \multicolumn{4}{c}{\textbf{ELTL}}\\ 
    \cmidrule{2-5} \cmidrule{7-10} \cmidrule{12-15} \cmidrule{17-20} 
                               &L      & F1   & Acc  & T    &&L      & F1   & Acc  & RT   &&L     &F1 & Acc & T  &&L&F1  & Acc& T \\
    \textbf{C}              & ?     & ? & ? & ?  && ?     & ? & ? & ?  && ?     & * & ?  & ? && ?    & ?& ? &?\\
    \bottomrule
    \end{tabular}
    \label{table:family_results}
 \end{table*}


